Associative Alignment for Few-shot Image Classification

Few-shot image classification aims at training a model from only a few examples for each of the "novel" classes. This paper proposes the idea of associative alignment for leveraging part of the base data by aligning the novel training instances to the closely related ones in the base training set. This expands the size of the effective novel training set by adding extra "related base" instances to the few novel ones, thereby allowing a constructive fine-tuning. We propose two associative alignment strategies: 1) a metric-learning loss for minimizing the distance between related base samples and the centroid of novel instances in the feature space, and 2) a conditional adversarial alignment loss based on the Wasserstein distance. Experiments on four standard datasets and three backbones demonstrate that combining our centroid-based alignment loss results in absolute accuracy improvements of 4.4%, 1.2%, and 6.2% in 5-shot learning over the state of the art for object recognition, fine-grained classification, and cross-domain adaptation, respectively.

==> sec_baseline.tex <==
\section{Establishing a strong baseline} 
\label{sec:baseline}

Before evaluating our alignment strategy in sec.~\ref{sec:experiments}, we first establish a strong baseline for comparison by following the recent literature. In particular, we build on the work of Chen \emph{et al.}~\cite{chen2019closer} but incorporate episodic early stopping on the pre-training stage with a different loss function.

\subsection{Episodic early stopping} 
\label{sec:early-stopping}
A fixed number of epochs in the pre-training stage has been commonly used (e.g., \cite{chen2019closer,finn2017model,snell2017prototypical,vinyals2016matching}), but this might hamper performance when fine-tuning on novel classes. Using validation errror, we observe the necessary of early-stopping in pre-training phase. 
%
{\color{red} Please see supplementary material for episodic validation error plot}. 
%
%This is illustrated in fig.~\ref{fig:overfitting}, 
%
%which plots validation error after fine-tuning vs. the number of pre-training epochs. The ``cosmax'' function is used, with the entire network pre-trained on $\mathcal{X}^b$, and only the classification weights $\mathbf{W}$ fine-tuned on $\mathcal{X}^n$, as in~\cite{chen2019closer}. The decrease in accuracy over the epochs (after 150 epoch for 1-shot) shows that pre-training should not be conducted for a fixed number of epochs. 
We thus propose to make use of episodic early stopping on the validation categories at pre-training time, more specifically by stopping the training when the mean accuracy on the validation over a window of recent epochs starts to decrease. The best model in the window is selected as the final result.


\subsection{Classification loss functions} 
\label{sec:arcmax}

Deng \emph{et al.}~\cite{deng2018arcface} have shown that an additive angular margin (``arcmax'' hereafter) outperforms other metric learning algorithms for face recognition. The arcmax function has a metric learning property since it enforces a geodesic distance margin penalty on the normalized hypersphere, which we think can be beneficial for few-shot classification by helping keep classes cluster compact and well-separated. 

% Let $\mathbf{z}$ be the embedding representation of an example $\mathbf{x}$. 

% \todo{Has $\mathbf{z}$ been defined before? If not, it probably should? (ar)} 

Let $\mathbf{z} = f(\mathbf{x}|{\theta})$ be the representation of $\mathbf{x}$ in feature space. As per \cite{deng2018arcface}, we transform the logit as $\mathbf{w}_j^\top \mathbf{z} = \|\mathbf{w}_j \| \|\mathbf{z} \| \cos \varphi_j$, where $\varphi_j$ is the angle between $\mathbf{z}$ and $\mathbf{w}_j$, the $j$-{th} column in the weight matrix $\mathbf{W}$. Each weight $\|\mathbf{w}_j\| = 1$ by $l_2$ normalization. Arcmax adds an angular margin $m$ to the distributed examples on a hypersphere:  
%
\begin{equation}\label{eq:arcmax} 
  \mathcal{L}_{\mathrm{clf}} = 
 -\frac{1}{N} \sum_{i=1}^N \log \frac{\exp(s\cos (\varphi_{y_i}+m))}{\exp(s \cos (\varphi_{y_i}+m)) + \sum\limits_{\forall j\neq y_i} \exp(s \cos \varphi_j)} \,,\nonumber
\end{equation} 
%
where $s$ is the radius of the hypersphere on which feature embeddings are distributed, $N$ the number of examples, and $m$ and $s$ are hyperparameters (see sec.~\ref{sec:datasets-implementation}). The overall goal of the margin is to enforce inter-class discrepancy and intra-class compactness simultaneously.
%\begin{figure}[!t]
%\centering
%\includegraphics[scale=0.072]{figures/figure2_arc_cos_soft.pdf}
%\caption{Validation error after fine-tuning as a function of the number of pre-training base epochs on \textit{mini}-ImageNet with the cosmax loss function. Pre-training for a fixed number of iterations (here 400 as in \cite{chen2019closer}) may lead to overfitting the feature extraction on the base set. Each curve represents the average of 50 episodes. 
% Arcmax versus cosmax and softmax on validation set of \textit{mini}-ImageNet in 5-way, 1-shot scenario.  The same color represents an identical $k-$shot setup and encoder. Continuous lines represent arcmax. Dot and dash lines illustrate softmax and cosmax, respectively. Each curve presents an average of 50 episodes. 
%}
%\label{fig:overfitting}
%\end{figure} 


